PC-JeDi: Diffusion for Particle Cloud Generation in High Energy Physics

In this paper, we present a new method to efficiently generate jets in High Energy Physics called PC-JeDi. This method utilises score-based diffusion models in conjunction with transformers which are well suited to the task of generating jets as particle clouds due to their permutation equivariance. PC-JeDi achieves competitive performance with current state-of-the-art methods across several metrics that evaluate the quality of the generated jets. Although slower than other models, due to the large number of forward passes required by diffusion models, it is still substantially faster than traditional detailed simulation. Furthermore, PC-JeDi uses conditional generation to produce jets with a desired mass and transverse momentum for two different particles, top quarks and gluons.

==> preamble.tex <==
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{physics}
% \usepackage[a4paper]{geometry}

\usepackage[margin=0.7in]{geometry}
\usepackage{authblk}
\usepackage{tabularx}

\usepackage{url}
\usepackage{longtable}
\usepackage{multirow}
\usepackage[font=small,skip=0pt]{caption}
\usepackage[labelformat=simple]{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}

\usepackage[nodayofweek]{datetime}
\usepackage{enumerate}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[export]{adjustbox}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[pdftex,hidelinks]{hyperref}
\usepackage{bookmark}
% \usepackage[compat=1.1.0]{tikz-feynman}

\usepackage{float}
\usepackage[capitalise]{cleveref}

% \input{preamble-tikz.tex}

\setlength{\mathindent}{8ex}
\setlength{\parindent}{0pt}
\setlength{\parskip}{5pt}

\linespread{1.5}
% \renewcommand{\arraystretch}{1.5}
\frenchspacing

\hyphenation{ATLAS}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage[backend=biber,giveninits=true,doi=true,sorting=none,style=numeric-comp]{biblatex}
\DeclareFieldFormat[article]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[article]{title}{\textit{#1}\isdot}
\DeclareFieldFormat[unpublished]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[unpublished]{title}{\textit{#1}\isdot}
\DeclareFieldFormat[inproceedings]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[inproceedings]{title}{\textit{#1}\isdot}

\DeclareNameAlias{author}{family-given}

% This is all for adding line numbers to the draft
% \usepackage{lineno}
% \linenumbers
% \let\oldequation\equation
% \let\oldendequation\endequation
% \renewenvironment{equation}
%   {\linenomathNonumbers\oldequation}
%   {\oldendequation\endlinenomath}

% \addbibresource{bib/ATLAS.bib}
% \addbibresource{bib/CMS.bib}
% \addbibresource{bib/Extra.bib}
% \addbibresource{bib/HiggsSMrefs.bib}
% \addbibresource{bib/PubNotes.bib}
% \addbibresource{bib/myrefs.bib}
% \addbibresource{bib/rodem.bib}
% \addbibresource{bib/bibraine.bib}
\addbibresource{bib/biblio.bib}

